Backpropagating through Fr\'echet Inception Distance

The Fr\'echet Inception Distance (FID) has been used to evaluate hundreds of generative models. We introduce FastFID, which can efficiently train generative models with FID as a loss function. Using FID as an additional loss for Generative Adversarial Networks improves their FID.

==> sections/1_introduction.tex <==
\section{Introduction}
Generative modeling is a popular approach to unsupervised learning, with applications in, e.g., computer vision \cite{dcgan} and drug discovery \cite{moses}. 
A key difficulty for generative models is to evaluate their performance, i.e., how good is the generative model approximating the data distribution?

For images, it is best-practice to use the Fréchet Inception Distance (FID) \cite{fid}, which is currently used through-out the research community. 
Inspired by the popularity of FID when \emph{evaluating} generative models, we ask whether FID can also be used to \emph{train} generative models. To answer this question we identify two core problems. 

Firstly, while it is possible to backpropagete through FID, every single mini-batch computation takes around $10s$.
We mitigate this issue by introducing FastH which reduce the time to around $0.1s$. 

Second, we find that training generative models to minimize FID often leads to generative models that ``cheat'' FID by generating ``adversarial examples``. 
Perhaps surprisingly, we find that Generative Adversarial Networks surpass this issue because the discriminator automatically detects and penalize such ``cheating''. 

We find explicit minimization of FID consistently improves GANs, see Figure 1. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/frontpage.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


%Does models that explicitly minimize FID produce images of higher quality, or do they exploit the inner workings of the inception network? (fill right side with images, have 1 for each dcgan/sogan/logan, and then one with image that qualitatively demonstrate what FID helps with. This takes too long, so we introduce FastH which computes FID much faster. 

%After realizing minimization of FID makes sense, we used FID to fine-tune BIGGAN to attain SOTA performance. 

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{0.47\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/frontpage_noise.pdf}% Validation FID 33.8
%        \caption{Adversarial Noise}
%        \label{subfig:front_noise}
%    \end{subfigure}
%    \begin{subfigure}{0.47\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figures/frontpage_example.pdf}% Validation FID 1003.4
%        \caption{Adversarial Example}
%        \label{subfig:front_example}
%    \end{subfigure}
%    \caption{
%    First row is original noise (bad FID) and original data (good FID). 
%    Second row contains modified noise (good FID) and modifid data (bad FID). 
%    See \Cref{sec:adv} for details. }
%    \label{fig:front_page}
%\end{figure}

==> sections/3_fast_frechet_distance.tex <==


\section{Fast Fréchet Inception Distance}\label{sec:algo}
The FID between the model distribution $P_{model}$ and the real data distribution $P_{data}$ is computed as follows. 
Draw ``fake'' model samples $f_1,...,f_m\sim P_{model}$ and ``real'' data samples $r_1,...,r_n\sim P_{data}$.
Encode all samples $f_i$ and $r_i$ by computing activations $A(f_i)$ and $A(r_i)$ of the final layer of the pretrained Inception network~\cite{inception}. 
Compute the sample means $\mu_1,\mu_2$ and the sample covariance matrices $\Sigma_1, \Sigma_2$ of the activations $A(f_i), A(r_i)$. 
The FID is then the Wasserstein distance \cite{wasserstein} between the two multivariate normal distributions $N(\mu_1,\Sigma_1)$ and $N(\mu_2, \Sigma_2)$. 
\begin{equation}\label{equ:wasserstein}
    %W(N(\mu_1, \Sigma_1), N(\mu_2, \Sigma_2))^2= 
    ||\mu_1 - \mu_2||_2^2 + \tr(\Sigma_1) + \tr(\Sigma_2) - 2\cdot \tr( \sqrt{\Sigma_1\Sigma_2})
\end{equation}
For evaluation during training, the original implementation use $10000$ samples by default \cite{fid}. 
On our workstation,\footnote{RTX 2080 Ti with Intel Xeon Silver 4214 CPU @ 2.20GHz, computing FID on CelebA \cite{celeba} images using the following implementation of FID \url{https://github.com/hukkelas/pytorch-frechet-inception-distance} with precomputed Inception encodings of the real data. } this cause the FID evaluation to take approximately $20s$. 
Of the $20s$, it takes 
approximately $10s$ to compute Inception encodings and approximately $10s$ to compute $\tr(\sqrt{\Sigma_1\Sigma_2})$. 

The real data samples $r_1,...,r_n$ does not change \emph{during} training, so we only need to compute their Inception encodings once. 
The $10s$ spent computing the Inception encodings is only the time it takes to encode the fake model samples $f_1,...,f_m$. 
It is thus sufficient to reduce the number of fake samples $m$ to reduce the time spent computing Inception encodings.
For example, if we reduce $m$ from $10000$ to $128$ we reduce the time spent computing Inception encodings from $10s$ to $0.1s$. 
However, it still takes around $10s$ to compute $\tr(\sqrt{\Sigma_1\Sigma_2})$. 
FastFID mitigates this issue by efficiently computing $\tr(\sqrt{\Sigma_1\Sigma_2})$ without explicitly computing $\sqrt{\Sigma_1\Sigma_2}$. 
\Cref{subsec:prevalgo} outlines how previous work computed $ \sqrt{\Sigma_1\Sigma_2}$ and \Cref{subsec:ouralgo} introduce our novel algorithm that efficiently computes $\tr(\sqrt{\Sigma_1\Sigma_2})$. 

\subsection{Previous algorithm } \label{subsec:prevalgo} % https://arxiv.org/pdf/1712.01034.pdf is O(d^^2 * convergence) 
The original FID implementation \cite{fid} computes $\tr(\sqrt{\Sigma_1\Sigma_2})$ by explicitly constructing $\sqrt{\Sigma_1\Sigma_2}$. 
The matrix square root is computed using \textsc{scipy.linalg.sqrtm} \cite{scipy} which implements an extension of the algorithm from \cite{sqrtm} which is rich in matrix-matrix operations \cite{scipysqrtm}. 
The algorithm starts by computing the following Schur decomposition. 
\begin{equation}\label{equ:schur}
    \Sigma_1\Sigma_2 = Q V Q^T\text{ where } Q^T=Q^{-1}\text{and }V\text{ is triangular. }
\end{equation}
The algorithm then computes a triangular matrix $U$ such that $U^2=V$ by exploiting the triangular structure of both $U$ and $V$. 
In particular, the triangular structure implies the following triangular equations $U_{ii}^2=V_{ii}$ and $U_{ii}U_{ij}+U_{ij}U_{jj}=V_{ij}-\sum_{k=i+1}^{j-1}U_{ik}U_{kj}$ \cite{scipysqrtm}. The equations can be solved wrt. $U$ one superdiagonal at a time. 
The resulting $U$ yields a matrix square root of the initial matrix. 
\begin{equation}
\label{equ:schur_sqrt}
    \sqrt{\Sigma_1\Sigma_2}=Q U Q^T
\end{equation}
\paragraph{Time Complexity. }
Computing the Schur decomposition of a $d\times d$ matrix $\Sigma_1\Sigma_2$ takes $O(d^3)$ time. 
The resulting triangular equations can then be solved wrt. $U$ in $O(d^3)$ time. 
The entire matrix square root computation then takes $O(d^3)$ time. 
The size of $d$ depends on the network that encodes the data. 
For example, FID uses the Inception network which has $d=2048$ while FCD uses the ChemNet network which has $d=512$. 
On our workstation, the different values of $d$ cause the square root computations to take approximately $10s$ for FID and $1s$ for FCD. % it is around 7s and .5s, I just think round gives less cognitive stain. 

\paragraph{Uniqueness. }
The matrix square root $\sqrt{M}$ is defined to be any matrix that satisfies $\sqrt{M}\sqrt{M}=M$. 
The square root of a matrix is in general not unique, i.e., some matrices have many square roots. 
The above algorithm does not necessarily find the same square root matrix if it is run several times, because 
the Schur decomposition is not unique. 
Furthermore, when computing $U_{ii}=\sqrt{T_{ii}}$ one has the freedom to choose both $\pm |\sqrt{T_{ii}}|$. The \textsc{scipy.linalg.sqrtm} implementation choose $U_{ii}=|\sqrt{T_{ii}}|$. 
Our implementation of the algorithm we present in \Cref{subsec:ouralgo} computes the trace $\tr(\sqrt{\Sigma_1\Sigma_2})$ such that it agrees with \textsc{scipy.linalg.sqrtm} up to numerical errors. 


\subsection{Our algorithm }\label{subsec:ouralgo}
This subsection presents an algorithm that computes $\tr(\sqrt{\Sigma_1\Sigma_2)}$ fast.
The high-level idea: construct a ``small'' matrix $M$ such that the eigenvalues $\lambda_i(M)$ satisfy $\sum_i|\sqrt{\lambda_i(M)}|=\tr(\sqrt{\Sigma_1\Sigma_2})$. 
Since $M$ is small, we can compute its eigenvalues faster than we can compute the matrix square root $\sqrt{\Sigma_1\Sigma_2}$. 

Let $X_1\in\R^{d\times m}$ be a matrix with columns $A(f_1),...,A(f_m)$, let $X_2\in\R^{d\times n}$ be a matrix with columns $A(r_1),...,A(r_n)$ and let $\mathbb{1}_{k}$ be the $1\times k$ all ones vector. 
The sample covariance matrices $\Sigma_1$ and $\Sigma_2$ can then be computed as follows:
\begin{equation}\label{equ:covmatrix} 
    \Sigma_i= C_i C_i^T, \quad\text{where}\quad 
    C_1=\frac{1}{\sqrt{m-1}}(X_1-\mu_1 \mathbb{1}_{m}) \quad\text{and} \quad 
    C_2=\frac{1}{\sqrt{n-1}}(X_2-\mu_2 \mathbb{1}_{n}) 
\end{equation}
This allows us to write $\Sigma_1\Sigma_2=C_1C_1^T C_2C_2^T$. 
Recall that the eigenvalues of $AB$ are equal to the eigenvalues of $BA$ if both $AB$ and $BA$ are square matrices \cite{eigfact}. 
The eigenvalues of the $d\times d$ matrix $C_1C_1^TC_2C_2^T$ are thus the same as the eigenvalues of the $m\times m$ matrix $M=C_1^TC_2C_2^TC_1$.
The matrix $M$ is small in the sense that we will use $m\ll d$, for example, for FID we often use $m=128$ fake samples while $d=2048$. 

We now show that $\sum_i|\sqrt{\lambda_i(M)}|=\tr(\sqrt{\Sigma_1\Sigma_2})$ if $\sqrt{\Sigma_1\Sigma_2}$ is computed by \textsc{scipy.linalg.sqrtm}. 
Since $\tr(\sqrt{\Sigma_1\Sigma_2})=\sum_i\lambda_i(\sqrt{\Sigma_1\Sigma_2})$ it is sufficient to show that the eigenvalues of $\sqrt{\Sigma_1\Sigma_2}$ are equal to the positive square root of the eigenvalues of $\Sigma_1\Sigma_2$, that is,  
$\lambda_i(\sqrt{\Sigma_1\Sigma_2})=|\sqrt{\lambda_i(\Sigma_1\Sigma_2)}|$.

Recall that $\sqrt{\Sigma_1\Sigma_2}=QUQ^T$ where $\Sigma_1\Sigma_2=QVQ^T$, $U^2=V$ and $U_{ii}^2=V_{ii}$. 
Since both $U$ and $V$ are triangular they have their eigenvalues on the diagonal, which means that $\lambda_i(\sqrt{\Sigma_1\Sigma_2})=U_{ii}=\sqrt{V_{ii}}=\sqrt{\lambda_i(\Sigma_1\Sigma_2)}$. 
Recall that \textsc{scipy.linalg.sqrtm} choose $U_{ii}=|\sqrt{V_{ii}}|$ and we get $\lambda_i(\sqrt{\Sigma_1\Sigma_2})=|\sqrt{\lambda_i(\Sigma_1\Sigma_2)}|$ as wanted. 
Note that even though the Schur decomposition $\Sigma_1\Sigma_2=QUQ^T$ is not unique, $U$ will always have the eigenvalues of $\Sigma_1\Sigma_2$ on its diagonal and thus preserve the trace. 
Putting everything together, we realize that 
$
\tr(\sqrt{\Sigma_1\Sigma_2})=\sum_{i=1}^{m-1} |\sqrt{\lambda_i(C_1^TC_2C_2^TC_1)}|$.

For completeness, we provide pseudo-code in \Cref{algo:pseudocode}.
The algorithm can be modified to compute FCD by simply changing the Inception network to the ChemNet network. 

\paragraph{Time Complexity.}
Computing $M=(C_1^TC_2)(C_2^TC_1)$ takes $O(mdn+m^2n)$ time. 
The eigenvalues of $M$ can be computed in $O(m^3)$ time, giving a total time complexity of $O(mdn+m^2n+m^3)$. 
If we use a large number of real samples $n\gg d$, we can precompute $\Sigma_2=C_2C_2^T$ and compute $M=C_1^T\Sigma_2C_1$ in $O(d^2 m)$ time, giving a total time complexity of $O(d^2m+m^3)$. 


\begin{algorithm}[h!]
   \caption{Fast Fréchet Inception Distance}
   \label{algo:pseudocode}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $f_1,...,f_m\sim P_{model}$, the Inception network $\text{Net}(x)$ and precomputed $\mu_2,C_2$. 
   \STATE 
   \STATE // Compute network activations 
   \STATE Compute $A(f_i)= \text{Net}(f_i)$ and let $X_1$ be a matrix with columns $A(f_1),...,A(f_m)$. %and $A(r_i) = \text{Net}(r_i)$
   %\COMMENT{\hfill $\triangleright \; O(dm^2)$} 
   \STATE 
   \STATE // Compute mean. 
   \STATE $\mu_1 = \frac{1}{m}\sum_{i=1}^m(X_1)_i $. 
   \STATE 
   \STATE // Compute trace of square root matrix. 
   \STATE $C_1=\frac{1}{\sqrt{m-1}}(X_i-\mu_i \mathbb{1})$  as in \Cref{equ:covmatrix}. 
   \STATE $S = \text{library.eigenvalues}( (C_1^TC_2) (C_2^TC_1) )$
   \STATE $\tr(\sqrt{\Sigma_1\Sigma_2})= \sum_{i=1}^{m-1}|\sqrt{S_i}|$
   \STATE 
   \STATE // Compute trace of both covariance matrices. 
   \STATE $\tr(\Sigma_1)=\sum_{i=1}^m \text{row}_i(C_1)^T\text{row}_i(C_1)$ 
   \STATE $\tr(\Sigma_2)=\sum_{i=1}^n \text{row}_i(C_2)^T\text{row}_i(C_2)$
   \STATE 
   \STATE \textbf{return} $||\mu_1-\mu_2||_2^2 + \tr{(\Sigma_1)} + \tr{(\Sigma_2)} - 2 \cdot \tr(\sqrt{\Sigma_1\Sigma_2})$
\end{algorithmic}
\end{algorithm}

\paragraph{Computing Gradients. }
If the network $\text{Net}(x)$ used in \Cref{algo:pseudocode} supports  gradients with respect to its input, as the Inception network does, it is possible to compute gradients with respect to the input samples $f_i$. 
If $f_i$ were constructed by a generative model, one can even compute gradients wrt. the parameters of the generative model. 
If \Cref{algo:pseudocode} is implemented with autograd support, e.g., through PyTorch \cite{pytorch} or TensorFlow \cite{tf}, these gradients are computed automatically. 
For example, we implemented \Cref{algo:pseudocode} in PyTorch and used autograd to compute gradients when constructing adversarial examples in \Cref{sec:adv}. 

\paragraph{Potential Further Speed-ups. } 
In this section, we have focused on decreasing the time consumption of $\tr(\sqrt{\Sigma_1\Sigma_2})$. 
As a result, the majority of the time consumption of \Cref{algo:pseudocode} is spent computing Inception encodings. 
The Inception encodings could be further speed up by, e.g., compressing \cite{compress} the used network at the cost of introducing some small error. 

\begin{figure}[b]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/exp_running_times.pdf}
    \caption{Comparison of \textsc{scipy.linalg.sqrtm} and \Cref{algo:pseudocode} for different batch sizes. Left: Time it takes to compute Fréchet Inception Distance. Middle: Time it takes to compute Fréchet ChemNet Distance. Right: Time it takes to compute trace of matrix square root.  }
    \label{fig:speed}
\end{figure}


%\subsection{Adaptive}
%main idea.  by the BNS formula a rank 1 update changes eigenvaleus so they are interleaved by the previous eigenvalue. 
%One can efficiently compute inverse products with $\Sigma + BB^T$ where $B$ is rank $K$ using woodbury formula. 
%This allows us to use inverse power iteration, which, given an initial guess of an eigenvalue, finds that eigenvalue with exponential convergence in distance between eigenvalues.  
%The inverse power iteration requires using the inverse matrix for different offsets; for each of these offsets we need to compute the matrix inversion, and there are roughly $d$ of thme. This gives $d$ matrix inversions of size $bs^3$ which obviously takes too long. 
%However, I think we can mend this by using woodbury formula on the matrix inversion itself. We want to compute $(I-B^T D B)^{-1}$ for $D=\Sigma - c\I$ where $c=\lambda_1, \lambda_2, ..., \lambda_d$. 
%
%I'm not that sure the woodbury thing will help us anymore, but I think one can do something else probably.;; the code is fast enough to beat the eigendecomposition; 128 points are updated in 0.045 seconds and full eigendecomp takes 2.48, this is 60 times faster. But the total number of updates is $2000/128=15$, so it is 4 times faster. But I think we can make it even faster, lol. 
%
%so this means, in practice, we will be able to beat eigendecomposition algorithm and find eigendecompositions a lot faster? that would be pretty cool! (we need a lot of enginneering to handle all these numerical errors) ;; the 25 power iterations takes only $0.003s$ compared to eigendecomposition which takes $2.48s$, 826 times faster! 
%
%Alternatively, one can make each rank one update sequentally, but this is just not good because then errors accumalte. 
%Errors can be brought down by keeping an exact adaptively comptued covariance matrix, and then, once in a while, computing the eigendecomposition. One might also make an algorithm that looks at the real thing and then figures out how to update the eigendecomposition if it is not too bad; maybe it is only a small rank away? 



\section{Experimental Performance of FastFID}
\label{sec:exp}
\subsection{Speed-Up}\label{subsec:pracspeedup}
In \Cref{sec:algo}, we presented a fast algorithm to compute $\tr(\sqrt{\Sigma_1\Sigma_2})$, which can be used to speed up the computation of both FID and FCD. 
In this subsection, we compare the running time of our PyTorch \cite{pytorch} implementation of \Cref{algo:pseudocode} against open-source
implementations.\footnote{See \textsc{scipy.linalg.sqrtm} from \cite{scipy}, \url{https://github.com/insilicomedicine/fcd_torch} and \url{https://github.com/hukkelas/pytorch-frechet-inception-distance} } 
The algorithms are compared as the number of different fake samples varies $m=256,128,...,8$. 

We used images from the CelebA dataset \cite{cifar} when timing FID. 
We used SMILES molecules from the MOSES dataset \cite{moses} when timing FCD. 
For both FID and FCD, we precomputed $\Sigma_2$ with $10000$ real samples. 
We also timed $\tr(\sqrt{C_1^T\Sigma_2C_1})$ in isolation, by using $\Sigma_2\in \R^{d\times d}$ with $N(0,1)$ entries and computed $C_1$ from \Cref{equ:covmatrix} where $X_1\in \R^{d\times n}$ has $N(0,1)$ entries. 
To make timings of $\tr(\sqrt{C_1^T\Sigma_2C_1})$ comparable with FID, we chose $d=2048$ so it matches the Inception network. 

For each $m$, we ran one warmup round and then repeated the experiment $100$ times. 
\Cref{fig:speed} plots average running time with standard deviation as error bars.\footnote{For our algorithm, we plot $[\mu-\sigma/2, \mu+\sigma]$ instead of $\mu\pm \sigma$ to avoid clutter caused by the logarithmic scaling. This means that the real running time of our algorithm is sometimes a little bit better than visualized. } 
The previous algorithm takes roughly the same amount of time for all $m$. 
This is expected since the matrix square root takes up most of the computation time, and the computation time does not depend on $m$. 
Our algorithm takes less time as $m$ decrease. 
This is expected since our algorithm takes $O(m^3+d^2m)$ time for precomputed $\Sigma_2$. 

For all $m$, our algorithm is at least $25$ times faster than the previous algorithms, and in some cases up to hundreds or even thousands of times faster. 
We emphasize that both algorithms were given the same task and computed the same thing, our algorithm was just faster. 





% make this into a subsection 
\subsection{Numerical Error } \label{subsec:numerror}
To investigate the numerical error of \Cref{algo:pseudocode} and \textsc{scipy.linalg.sqrtm}, we ran an experiment where the square root can easily be computed. 
If we choose $C_1=C_2$ then $C_1C_1^TC_2C_2^T=(C_1C_1^T)^2$ is positive semi-definite and has an unique positive semi-definite square root $\sqrt{(C_1C_1^T)^2}=C_1C_1^T$. 
Furthermore, it is exactly this positive semi-definite square root \textsc{scipy.linalg.sqrtm} computes, since the implementation chooses the positive eigenvalues $U_{ii}=|\sqrt{V_{ii}}|$ (see \Cref{subsec:prevalgo} for details). 
We can then investigate the numerical errors by comparing the ground truth $\tr(C_1C_1^T)$ with the result from both \Cref{algo:pseudocode} and \textsc{scipy.linalg.sqrtm}. 
To amplify the numerical errors we used 32-bit floating points instead of 64-bit floating points. 

The experiment was repeated for $m=32,64,128,256$ number of fake samples, were $C_1$ was computed as done in \Cref{subsec:pracspeedup}. 
We report the ground truth $\tr(C_1C_1^T)$ and the absolute numerical error caused by \Cref{algo:pseudocode} and \textsc{scipy.linalg.sqrtm}, e.g., we report $|\tr(C_1C_1^T)-\tr(\textsc{scipy.linalg.sqrtm}(C_1C_1^TC_1C_1^T))|$. 
See results in \Cref{fig:numerror}. 
The numerical error of \Cref{algo:pseudocode} is at least $1000$ times smaller than that of \textsc{scipy.linalg.sqrtm}. 
We suspect \Cref{algo:pseudocode} is more numerically stable because it computes eigenvalues of a ``small'' $m\times m$ matrix instead of computing a Schur decomposition of the ``full'' $d\times d$ matrix. 

%\input{tables/numerical_errors_simple}
% \input{tables/numerical_errors}

\section{Improved Models or Adversarial Attacks?}
We found that optimization of FID allows us to make adversarial examples, i.e., explain (see Appendix for details). If this is possible, one might be scared that generative models simply learn to make adversarial examples. As a matter of fact, we found that training normalizing flows to simultaneously minimize FID leads to this error mode (see Figure ...). 

To our surprise, we did not experience this failure mode in GANs. In Sec 4.1 we attempt to clarify this behaviour. In 4.2 we attempt to interpret what it means to augment GANs with an generator, and which impact this has on training relative to plain GAN training. ?FIDAN?

\subsection{Classifiability Experiments}
Make further experiments with classifiabilty of cheating. 

\subsection{Interpreting the loss}
batch dependency on loss. 

note the loss from normal discriminator are independent for each training example. For example, the gradient is computed by bla, bly. 

$$...$$

This has the disadvantage that the discriminator can not penalize the generator if it produces the same samples. On the other hand, the FID computes blabla, so it is capable of penalizing such behavior! 

$$ ...$$$ 


%\subsection{Saliency Maps}
%What does gradients from discriminator and Inception network tell the generator? If we make adversarial examples we can make images attain good fid, which indicates the samples cheat the inception network. It is also possible to cheat the Inception network, so the question remains, does this actually happen?
%%
%Image showing gradient from generator and discriminator. 

%\subsection{Covariates}


%\section{Efficiently Evaluating Generative Models During Training}\label{sec:eval}
%\subsection{Fréchet Inception Distance}
%It can be hard to determine whether a generative model improves during training. 
%This is particularly difficult for GANs, where one does not have a single numeric value that measures error. 
%For example, consider left plot in \Cref{fig:dcgan}, which displays the error of discriminator/generator during training of a DCGAN \cite{dcgan} on CelebA \cite{celeba} at $64\times64$ resolution. 
%This looks quite different to supervised error functions like mean squared error, which typically drops steadily during training. 
%Both the discriminator error and the generator error has no clear interpretation. 
%This makes it difficult to determine whether training improves the performance of the generator.
%
%To mitigate this issue, \cite{fid} used FID to evaluate a DCGAN \cite{dcgan} during training. 
%We similarly computed FID every $10$ mini-batch updates using $m=10000$, see the right plot in \Cref{fig:dcgan}.\footnote{The source-code from \cite{fid} use $m=10000$ by default, see \url{https://github.com/bioinf-jku/TTUR/blob/d4baae8c095876c01c032c3c53d5542b69887a9b/DCGAN_FID_batched/model.py\#L32}. 
%However, \cite{fid} report training FID since they precompute activations on the entire training set. 
%To take overfitting into account, we use a validation set of size $n=10000$ and precompute activations on the validation set. }
%The FID drops steadily during training, which indicates that training does indeed improve the performance of the generator, at least as measured by FID. 
%However, computing FID with $m=10000$ is computationally expensive. 
%Each FID computation took at least $20s$, while a single mini-batch update of the DCGAN took $0.09s$. 
%This means the FID computations took at least $20$ \emph{times} the training time, even though we only computed FID once every $10$ iterations.
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\textwidth]{figures/exp_gan_fid.png}
%    \caption{Left: discriminator and generator error when training DCGAN \cite{dcgan} on CelebA \cite{celeba}. 
%    Based on the error curves, it is difficult to determine whether (and how much) the generator is improving. 
%    Right: FID during training of DCGAN, FID consistently drops which indicates training does improve the generator. }
%    \label{fig:dcgan}
%\end{figure}
%To speed up the evaluation, we computed FID with \Cref{algo:pseudocode} using just $m=128$ fake samples, while still using the $n=10000$ precomputed activations on the validation set.
%The resulting FID computation took $0.2s$, at least $100$ times faster. 
%As a result, the FID computations took no more than $0.25$ \emph{times} the training time. 
%
%Let $FID_m$ denote FID evaluated with $m$ fake samples. 
%We plot both $FID_{128}$ and $FID_{10^4}$ during training of the DCGAN in \Cref{fig:loss}. 
%The left plot shows both FIDs during the first epoch (1500 mini-batch updates). 
%Both FIDs drop during training, and they qualitatively appear to be very similar. 
%The middle plot shows that both FID losses behave similarly throughout training. 
%
%To quantify the error we get by using $FID_{128}$ instead of $FID_{10^4}$, we attempt to measure how good $FID_{128}$ is at predicting $FID_{10^4}$. 
%For simplicity, we fitted a linear regression model $f(FID_{128})=a\cdot FID_{128}+b$ to approximate $FID_{10^4}$.
%The linear regression model solves to $f(x)=1.086x-54.165$ which attains correlation coefficient $r=0.995$ and a mean squared error of $0.0032$. 
%The right plot in \Cref{fig:loss} shows $FID_{128}$ on x-axis and $FID_{10^4}$ on y-axis and the linear regression model.
%
%The linear model suggests that the computed $FID_{10^4}$ and $FID_{128}$ are roughly related by an offset. 
%It thus seems reasonable to use $FID_{128}$ as a measure of relative generative improvement during training. 
%We emphasize that the $100\times$ speed-up typically makes the difference as to whether such quantitative evaluation is practically feasible or not. 
%One of the main difficulties when debugging and experimenting with GANs, is the lack of a single numeric measure of generative performance that can be frequently evaluated at a low cost, this is now possible with $FID_{128}$ using \Cref{algo:pseudocode}.  
%

%Interpret the linear model. What does this actually mean, we'll, it just looks like it is consistently $40$ FID off later on due to using less samples. 
%This can still be used to measure relative model improvement.
%We believe a $100\times$ speed-up is very useful while debugging model, trying out new ideas as GANs is an area fast testing of ideas is important, and current FID computation is too slow to allow that. emphasize data behaves more linearly in start, indicating the earlier we use this trick the more sense it makes. 

%The supplementary material contains PyTorch code that can compute $FID_{m}$ in one line of code. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=1\textwidth]{figures/loss.png}
%    \caption{Comparison of FID computed with $m=128$ and $m=10^4$ when evaluating DCGAN \cite{dcgan} trained on CelebA \cite{celeba} at resolution 64x64. Left: First 1600 mini-batch updates, most peaks co-occur. Middle: Training throughout 10 epochs.  
%    Right: Relationship between $FID$ evaluated with $m=128$ and $m=10^4$ fake samples, and the best linear fit $r=0.995$.  }
%    \label{fig:loss}
%\end{figure}
%
%
%\subsection{Frechet ChémNet Distance}
%On image data it is often possible for humans to qualitatively evaluate whether model samples improve during the early stages of training. 
%However, it seems harder for humans to carry out such qualitative assessment when the generated samples are, e.g., molecules. 
%This motivates the need for quantitative evaluation of molecules during training of generative models. 
%In this section, we demonstrate that \Cref{algo:pseudocode} also allows efficient computation of FCD. 
%For simplicity, we retrained the Variational AutoEncoder from \cite{moses} on the MOSES dataset and compared $FCD_{128}$ against $FCD_{10^4}$. 
%The results are visualized in \Cref{fig:loss_fcd} following the same structure as \Cref{fig:loss}. 
%It took around $1.87s$ to compute $FCD_{10^4}$ and only $0.055s$ to compute $FCD_{128}$, at least $30$ times faster. 
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=1\textwidth]{figures/loss_fcd.png}
%    \caption{Comparison of FCD computed with $m=128$ and $m=10^4$ when evaluating VAE trained on MOSES \cite{moses}. Left: First $1000$ mini-batch updates, most peaks co-occur. Middle: Training throughout $10000$ mini-batch updates.  
%    Right: Relationship between $FCD$ evaluated with $m=128$ and $m=10^4$ fake samples, and the best linear fit $r=0.996$.  }
%    \label{fig:loss_fcd}
%\end{figure}

\begin{figure}[b]
    \centering
    \begin{subfigure}{0.435\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/adversarial_losses_noise.pdf}
        \caption{Adversarial Noise}
        \label{subfig:adversarial_noise_loss}
    \end{subfigure}
    \begin{subfigure}{0.435\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/adversarial_losses_examples.pdf}
        \caption{Adversarial Examples}
        \label{subfig:adversarial_example_loss}
    \end{subfigure}
    \caption{FID loss curves for training adversarial examples. Validation and training loss are so close the lines overlap. (a) is loss corresponding to the fakes of \Cref{subfig:front_example} and right plot is loss for \Cref{subfig:front_noise}.}
    \label{fig:adversarial_losses}
\end{figure}

\clearpage 
\clearpage 
\clearpage 
\section{Appendix: Adversarial Examples}\label{sec:adv}
Previous work showed that it is possible to make images that fool neural network classifiers~\cite{panda}. 
One well know example makes an imperceptible modification to a correctly classified input image of a panda by adding a small vector of ``noise,'' which fools the classifier to predict the new input as a gibbon with high confidence~\cite{panda}. 

What would adversarial examples be for FID?
Here, we present two types. 
First, images that perceptibly look like random noise but attain good FID, denoted ``adversarial noise for FID.''
For an example, see the second row of \Cref{subfig:front_noise}. 
Second, images that perceptibly look real but attain a bad FID, denoted ``adversarial examples for FID.'' 
For an example, see the second row of \Cref{subfig:front_example}. 
Together, these two types of adversarial attacks show that it is possible to fool the FID. %\fh{Maybe add teaser for the network below that actually does fool FID}.

A simple way to make an adversarial input, being noise or a natural looking image, is to optimize $FID(z)$ by gradient updates from some starting point $z$.
We take $z$ to be samples from either random noise vectors $z \sim  N(0, 1)$ or random samples from the CelebA dataset~\cite{celeba}. To ensure that generated samples remain valid, i.e., in the range $[0; 1]$, under gradient updates, we apply the sigmoid function to the adversarial noise and clip values of adversarial examples.
To compute FID during training, we have pre-computed that statistics for a training set of 190 thousand samples and a validation set of ten thousand samples. 
We optimize the same batch of 64 samples to either maximize or minimize FID.
Note that the reported $FID_{64}$ is biased in the sense that it is an upper bound of $FID_{10^4}$. 
This bias means that the adversarial noise may have a better (lower) $FID_{10^4}$ since it is no more than $FID_{64}$. 
On the other hand, it means that the adversarial examples may be worse (lower). % since $FID_{10^4}$ %while the bias means that the adversarial noise are better The bias of adversarial noise (examples) means that it is better (worse). 
%This means that the FID of the adversarial examples is biased to be worse than the reported FID, while the FID of the adversarial noise is biased to be better FID than reported. 

\paragraph{Adversarial Noise for FID. }
\Cref{subfig:adversarial_noise_loss} depicts the training and validation loss during 500 gradient steps on a batch of noise.
The validation loss reaches an FID of 42.6 after 500 steps, as indicated by the gray dashed line.
In \Cref{subfig:front_noise}, one can compare random samples from the initial random batch of noise, which has a validation FID of 463.9, and the same samples but after the 500 gradient steps. 
The produced adversarial noise still visually looks like random noise but attains a low FID.

\paragraph{Adversarial examples for FID. }
\Cref{subfig:adversarial_example_loss} shows the training and validation loss during 200 gradient steps on a random sample of 64 real images from the CelebA data set.
After 200 steps, the validation FID is 9901.1, as indicated by the dashed grey line. 
Again, for a comparison between original samples and optimized samples, see \Cref{subfig:front_example}.



% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/adversarial_losses.pdf}}
%     \caption{FID loss curves for training adversarial examples. Left plot is loss corresponding to the fakes of Figure \fh{1.a} and right plot is loss for Figure \fh{1.b}.}
%     \label{fig:my_label}
% \end{figure}

% alternatively, we could have used glow to encode the image and then when decoding optimize the parameters of glow as in th previous section. But I don't think we need that. 

% \begin{figure}[t]
%     \centering
%     % \begin{subfigure}{0.48\textwidth}
%     %     \includegraphics[width=\textwidth]{figures/adversarial_example_loss.png}
%     % \end{subfigure}
%     % \begin{subfigure}{0.48\textwidth}
%     %     \includegraphics[width=\textwidth]{figures/adversarial_examples.png}
%     % \end{subfigure}
%     \includegraphics[width=\textwidth]{figures/adversarial_noise.pdf}
%     \caption{We can train samples to attain good FID against real data without resembling real data. Left: loss during training of adversarial examples, they reach around FID 40 (marked by the dashed grey line). This is an upperbound, since we use small mini-batcth, the real value could be better. PCGAN attain FID around 7 with way larger images.}
%     \label{fig:adversarial_noise}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/adversarial_examples.pdf}
%     \caption{Adversarial Examples for FID. Plot on the left depicts FID computed between minibatches of adversarial examples and real examples. Batchsizes are 128. Adversarial Examples after 100 iterations are shown in the right plot. \fh{The FID for the real images in between was $\sim 62$ before doing gradient ascent. This is a bit higher than Figure 3?} Maybe this is because difference in resolution; F.3 used 32x32 and yours are definitely higher resolution. }
%     \label{fig:adversarial_example}
% \end{figure}

%\section{Fréchet Inception Adversarial Examples}

%Train adversarial examples on celeba? 
%As a sanity check we trained Glow \cite{glow} on CelebA \cite{celeba} at 64x64 resolution, while computing FID at each iteration. 
%As expected, training cause both nll and fid to drop, see blue plot \Cref{fig:adversarial}.  
%We then train the same model augmented with the FID loss. 
%The resulting model attains roughly the same nll, but quickly attains a substantially better FID score, see gray plot in \Cref{fig:adversarial}. 
%
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\textwidth]{figures/exp_adversarial_loss.png}
%    \caption{Caption}
%    \label{fig:adversarial_loss}
%\end{figure}
%
%This drop in loss is caused by a type of examples the Glow network generates to adversarially fool the Inception network. 
%In particular, the images are high level noise with a bright noise on the border, see \Cref{fig:adversarial_examples} for an example. 
%
%To the best of our, this are the first adversarial examples trained specifically for FID. 
%However, from the perspective of training a generative model, such examples are highly undersirable. 
%Further investigation showed that these examples are not roboust to data augmentation techniques like rotation. 
%In other words, the adversarial examples are noise that get good/low FID by fooloing the Inception network, however, if we rotate them, they no longer fool the Inception network and they get a bad/high FID. 
%\begin{figure}[h]
%    \centering
  %  \includegraphics[width=\textwidth]{figures/exp_adversarial_examples.png}
  %  \caption{Caption}
%    \label{fig:adversarial_examples}
%\end{figure}
%%
%%%%

==> sections/4_evaluate.tex <==


\section{Evaluating Generative Models with FastFLD}\label{sec:eval}
It can be hard to debug generative models during training, in particular, it can be hard to debug GANs. Is the generative model even improving? For example, consider left plot in \Cref{fig:dcgan}, that displays the loss of discriminator/generator during training. It is hard to determine if training improves generative performance. However, if we look at right plot of \Cref{fig:dcgan}, we see FID drop, which makes us more confident that training improves the generative model. 

This type of evalaution was introduced by \cite{fid}, who e.g. evaluated a DCGAN model by computing FID every 1000 updates with $m=5000$ examples. 
\Cref{algo:pseudocode} allows us to decrease computation time and evaluate the model more frequently. 
In particular, we trained a DCGAN on celebA 64x64 with $m=128$ and evaluated the model every $10$ mini-batch updates\footnote{For simplicity we report training FID. }.
The result was used to create \Cref{fig:dcgan} as explained above. 

How can we justify the use of $m=128$ ? refer to previous section. 
As discussed in \Cref{sec:fiderror} we use a mini-batch size $m=128$ to and report FID every 10 mini-batch updates. 

We similarly demonstrate the use on MOSES with FCD, see \Cref{fig:aae} 


%Since the main issue is measuring progress during training, we report training FID computing on the same mini-batch against generated fakes; the main concern is that optimization improves loss, i.e., underfitting, which can be measured by training FID, not overfitting, which would require us to measure FID on a test/validation set. 

%Using our algorithm one can efficiently get FID /FCD loss during trainig . 
%\textbf{TODO} I think this has previously been done by someone with normal FID which is slow, even the original FID article, but probably only each epoch or something; mention that we now get measurements more often.


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/exp_gan_fid.png}
    \caption{Left: discriminator and generator loss when training DCGAN \cite{dcgan} on CelebA. Based on the loss curves, it is difficult to determine whether (and how much) the generator is improving. Right: mini-batch FID during training of DCGAN, FID consistently drops which means training does improve the generator. }
    \label{fig:dcgan}
\end{figure}

The supplementary contains PyTorch code that efficiently computes FID/FCD with just one line of code. 
Upon publication, we will make the code available to the public. 
%We plan to make the code available to the public upon publication. we plan to make publically available to efficiently measure performance of GAN with just one line of code, installed with PIP. 
%FID takes $?gb$ memory and $?s$ to evaluate and FCD takes $?$ memory and $?s$ time. \textbf{todo: measure how much this actually is} 

\textbf{I'm retraining the AAE model from moses; it looks like it doesn't really learn anything the first 15 epochs. It later halves learning rate each 20 epochs. I think this will be a good example where we can see what happens, then maybe by just chaning the learning rate, train the same model faster. }  % talk with the other guys, set up a Skype meeting. 
\textbf{to emphasize the FCD is working, we might show the FID decreasing steadily with the VAE model} 

\textbf{todo: compute only FCD on SMILES samples that parse} 



==> sections/5_adversarial.tex <==
\section{Adversarial Examples}\label{sec:adv}
Previous work showed that it is possible to make images that fool networks~\cite{panda}. 
One well know example is modifying a correctly classified input image of a panda by adding an imperceptibly small vector of ``noise,'' which fools the classifier to predict the new input as a gibbon with high confidence. 

What would adversarial examples be for FID?
Here, we present two types. 
First, images that perceptibly looks like random noise but attains good FID, denoted ``adversarial noise for FID.'' 
Second, images that perceptibly looks real but attains a bad FID, denoted ``adversarial examples for FID.'' 
Together, these two types of adversarial attacks questions the trustworthiness of the FID.

\paragraph{Adversarial Noise for FID. }
To make an adversarial example, one would normally minimize $FID(z)$ by gradient updates on some random input vector $z \sim N(0, 1)$.
However, we found optimization to progress faster by using the DCGAN from previous section and optimizing $FID(G_\Theta(z))$ wrt. the parameters $\Theta$ of the DCGAN.  
Using this method, we get an FID less than $40$ on minibatches of size 256 with the examples shown in the right plot of \Cref{fig:adversarial_noise}. 
Note how the experiment from \Cref{sec:minifid} indicate, that 40 is actually an upper bound on the real FID, since it was only computed for batches of size 256 here.
One might also suspect that we the comparison batch of real images is just overfitted by $G_\Theta$. For this reason, we include a validation FID, which is computed between $z$ and an unseen batch of 256 samples. 

% The fact that we computed FID on a mini-batch makes the FID an upperbound, this means that the real FID of the fakes would actually be lower! (we computed it wrt mini-batches of real data, so I would expect it to generalize well alos; it got 42 befre seeing entire dataset; and 34 a bit later, which might be overfit. 

% \url{ https://www.researchgate.net/figure/Frechet-Inception-Distance-and-Inception-Score-on-CelebA-and-CIFAR-10_tbl2_329234493 }

%\paragraph{Adversarial examples for FID. }
%To obtain adversarial examples for FID, we took an initial batch of 128 real images as our starting point $z \sim P_{data}$ and did gradient ascent on $FID(z)$.
%For a fair comparison, we computed the loss against one batch of samples and validated the FID score on an independent batch, not used for training.
%In \Cref{fig:adversarial_example}, we demonstarate how 200 gradient steps obtaines an FID of more than 10,000, while perceptually retaining  the original images.
%In comparison, note from \Cref{fig:adversarial_noise} how random noise attains an FID of roughly 350. 
%
% alternatively, we could have used glow to encode the image and then when decoding optimize the parameters of glow as in th previous section. But I don't think we need that. 

%\begin{figure}[t]
%    \centering
%    % \begin{subfigure}{0.48\textwidth}
%    %     \includegraphics[width=\textwidth]{figures/adversarial_example_loss.png}
%    % \end{subfigure}
%    % \begin{subfigure}{0.48\textwidth}
%    %     \includegraphics[width=\textwidth]{figures/adversarial_examples.png}
%    % \end{subfigure}
%    \includegraphics[width=\textwidth]{figures/adversarial_noise.pdf}
%    \caption{We can train samples to attain good FID against real data without resembling real data. Left: loss during training of adversarial examples, they reach around FID 40 (marked by the dashed grey line). This is an upperbound, since we use small mini-batcth, the real value could be better. PCGAN attain FID around 7 with way larger images.}
%    \label{fig:adversarial_noise}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\textwidth]{figures/adversarial_examples.pdf}
%    \caption{Adversarial Examples for FID. Plot on the left depicts FID computed between minibatches of adversarial examples and real examples. Batchsizes are 128. Adversarial Examples after 100 iterations are shown in the right plot. \fh{The FID for the real images in between was $\sim 62$ before doing gradient ascent. This is a bit higher than Figure 3?} Maybe this is because difference in resolution; F.3 used 32x32 and yours are definitely higher resolution. }
%    \label{fig:adversarial_example}
%\end{figure}
%
%%\section{Fréchet Inception Adversarial Examples}
%
%%Train adversarial examples on celeba? 
%%As a sanity check we trained Glow \cite{glow} on CelebA \cite{celeba} at 64x64 resolution, while computing FID at each iteration. 
%%As expected, training cause both nll and fid to drop, see blue plot \Cref{fig:adversarial}.  
%%We then train the same model augmented with the FID loss. 
%%The resulting model attains roughly the same nll, but quickly attains a substantially better FID score, see gray plot in \Cref{fig:adversarial}. 
%%
%%\begin{figure}[h]
%%    \centering
%%    \includegraphics[width=\textwidth]{figures/exp_adversarial_loss.png}
%%    \caption{Caption}
%%    \label{fig:adversarial_loss}
%%\end{figure}
%%
%This drop in loss is caused by a type of examples the Glow network generates to adversarially fool the Inception network. 
%%In particular, the images are high level noise with a bright noise on the border, see \Cref{fig:adversarial_examples} for an example. 
%%
%%%To the best of our, this are the first adversarial examples trained specifically for FID. 
%%However, from the perspective of training a generative model, such examples are highly undersirable. 
%%Further investigation showed that these examples are not roboust to data augmentation techniques like rotation. 
%%In other words, the adversarial examples are noise that get good/low FID by fooloing the Inception network, however, if we rotate them, they no longer fool the Inception network and they get a bad/high FID. 
%%\begin{figure}[h]
%%    \centering
  %  \includegraphics[width=\textwidth]{figures/exp_adversarial_examples.png}
%  %  \caption{Caption}
%    \label{fig:adversarial_examples}
%%\end{figure}
%%%
%%%%%
%
%%\section{Beyond SRemoving Supervision; this might be an aritcle itself; use a self-supervised network to trian generative using FID like measures. }
%%%The inception and ChemNet Networks are both trained supervised. 
%%However, this framework does not need the encoding network to be traind in a particular way. 
%%The encoding network could be any network that approximately outputs a normal distribution. 
%%For example, the encoder/inference part of a VAE. 
%The encoding part of a normalizing flow. 
%Network traind with self supervision, enforcing normality on the encodings, perhaps with batch norm as done in inception. 
%
%\section{Underconstrained} 
%Infinitely many models share the same likelyhood but represent almost aritrarily different distributions. 
%Adding the FID loss is a way of communicating that we care about images looking like ImageNet biased towards convolutions.% 

==> sections/6_train.tex <==
%\section{Fréchet Inception Distance as an Auxillary Loss}
\section{Negative Log Likelihood and Fréchet Inception Distances}\label{sec:aug}
In \Cref{sec:adv}, we demonstrated that it is easy to construct adversarial examples for FID. 
Consider training a generative model to minimize FID. 
This might give undesirable results because the generative model could ``cheat'' by generating adversarial examples \fh{noise?} for FID \fh{[We need to be careful here because we in \Cref{sec:adv} call samples ``adversarial examples'' when they look real but get bad FID, which is not the case here]}. 
To prevent the generaive model from generating adversarial examples, we train a generative model to minimize NLL and FID, simultaneously. 
The hope is that the NLL loss makes it harder for the model to cheat the FID loss, while the FID loss encourages the generative model to produce perceptually better images. 

%In this section we demonstrate how to circumvent this failure mode using FID as an auxillarby using the "FID error" estimates from \Cref{sec:minifid}. 

To allow NLL training, we use a Normalizing Flow \cite{nf} called Glow \cite{glow}. 
The model is trained on CelebA at a $32\times 32$ resolution in three different ways. 
NLL-Glow: trained normally to minimize NLL. 
FID-Glow: trained to minimize NLL and FID simultaneously. 
FID*-Glow: trained to minimize NLL and FID, but, as we explain next, we limit the use of the FID loss.

We use an open-source
implementation of Glow.\footnote{https://github.com/chrischute/glow}
The implementations default batch-size is $64$, so we also used $m=64$ samples to compute FID. 
The FID between two CelebA batches of size $64$ is $96$, this is what we called the ``FID error'' in  see \Cref{sec:minifid}. 
If we trained FID*-Glow to attain an FID below the FID error, our FID estimate would claim that generated data is closer to real data than real data is to real data. 
This seems unreasonable. 
We therefore only perform gradient updates wrt. FID as long as FID is lower\fh{[above right?]} than 96. See training FID/NLL in \Cref{fig:exp_celeba}. 

\paragraph{NLL-Glow. }Training NLL-Glow decrease its NLL. 
The FID also decrease (improve) during training. 
In particular, FID reaches around 99 at the end of training, which is just larger than the FID error $96\pm 2.6$. 
This means that the mini-batch FID computation is barely capable of telling us real data is more similar to real data, than generated samples is to real data. 

\paragraph{FID-Glow. }Perharps surprisingly, adding FID as an auxillary loss did not negatively impact the attained NLL. FID-Glow and NLL-Glow attain almost indistinguishable NLL during training. 
FID-Glow quickly attains an FID lower than NLL-Glow. 
When training finish, FID-Glow has an FID of 73 compared to 99 of NLL-Glow, a substantial improvement. 

However, the FID of 73 is way below the the ``FID error'' of 96. 
This means that the mini-batch FID estimates the generated samples are closer to real data, than real data is to real data. 
This indicates that the generative model probably learned to cheat the Inception network. 
This can be qualitatively verified by plotting the generated images \Cref{fig:fakes}. 

\paragraph{FID*-Glow. }
FID*-Glow manages to attain a low FID fast, but does not have access to gradients from the Inception network when its FID is below the ``FID error.''
It ends up with a mini-batch FID of $89$ without producing adversarial images like FID-Glow. 
This is a large improvement by simply changing the loss function. 
To check the improvement, we computed the FID at the end of training with $m=3000$ as usually done with CelebA; NLL-Glow attained $28.6$ and FID*-Glow atain FID of $19.5$.  % i actually used 3008=47*64
The generated samples are globally very similar, however, there are small differences like tan or background; see \Cref{fig:fakes}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/exp_celeb_loss.png}
    \caption{Training loss}
    \label{fig:exp_celeba}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{fakes_nll.png}
    \hspace{.5cm} 
    \includegraphics[width=0.3\textwidth]{fakes_fid.png}
    \hspace{.5cm} 
    \includegraphics[width=0.3\textwidth]{fakes_fid'.png}
    \caption{Generated samples. Left: FID-Glow. Middle: NLL-Glow. Right: FID*-Glow. Perhaps surprisingly, all samples are generated by models with the same NLL. }
    \label{fig:fakes}
\end{figure}

\textbf{Retrain everything and report validation loss. } 



%\paragraph{Tricks for Training}
%Initially, training produced startkly more wrose looking adversarial examples, see \Cref{}. 
%These examples achieved very good FID, however, they are essentially loss. 
%This was fixed by adopting data augmentation to the generated samples before computing FID; simple random 15 degree rotation and random flips solved the issue. 

%Gradient clipping of nll was not needed, but we used gradient clipping of FID of +-1. 

%During training we found it vital to take a step in the direction of nll and then afterwards take a step in fid, instead of taking both steps simultaneously. 

%The inception network consumes a lot of memory, especially when we need to simultaneously have a larger batch size. To scale to 256 batch-size we used gradient checkpointing of the Glow model and the inception network, computing FID activations in smaller 'mini-batches' of size 32. 


%\paragraph{Extending to FCD. }The Frechet ChemNet Distance uses one-hot encoding and tensor2string which are both discrete operations without gradients. In \cite{moses} they point out that one can circumvent this by A,B,C, this consistutes an interesting direction for future research. 


%\section{Redefining Fréchet Like Distances}
%They are defined wrong, find a way of making it work by e.g. taking the largest value so the model is demonstrated in the way it does the worst. 
%We might be able to demonstrate that the FID of random noise is 0 to everything if we compute the FID by exploiting the many matrix square roots. 


\section{Related Work}
Fréchet Inception Distance \cite{fid} was introduced to evaluate samples generate generative models. This was later extended to molecuules by \cite{fcd}. 
Other frechet like distances ...? 

\paragraph{Evaluation During Training}
FLD has been used to evaluate networks during trainig, this was even done in the initial FID paper. 
In this paper we bring down the cost of evaluating FID on a mini-batch during training. 
This does reduce performance, but we found it to be useful for comparing a model to itself, whereas comparing different models larger batch-sizes should be used. 

\paragraph{Previous Attempts at Speeding Up FID}
Previous work on speeding up FID like the official tensorflow implementation \cite{tfgan} attempt to circumvent matrix square root by (1) only computing mean difference $||\mu_1-\mu_2||$ or (2) only use diagonal of covarianec matrix. 
In this article we present a more principled approach that computes the same thing as the original algorithm, however, much faster for smaller mini-batches. 

\paragraph{Adversarial Examples and Training} To the best of our knowledge no previous work has sucesfully constructed adversarial exampels for FID or used FID as an auxillary loss. 

%\textbf{todo: } try to find previous article where they use FID to evaluate model; I THINK THEY DO THIS IN THE ARTICLE THAT INTRODUCES FID \cite{fid}. THen say they had to do it not that often, cause slow; in practice (cite tensorflow) people used heuristics like only computing means or diagonal covariance \cite{} \footnote{blabla.. they do something, which is $O(d^3)$ }. 


%Evaluation of generative models is difficult. 
%Most measures has some flaws, Likelihood based comparison has flaw \cite{}, FID has issue, for an overview see X. 

%In practice, most people are 


related work try to speed up by only comparing means \url{https://github.com/rockchip-linux/tensorflow/blob/master/tensorflow/contrib/gan/python/eval/python/classifier_metrics_impl.py} 


they even have a diagonal variant and write that this speeds up from O(n) to O($n^2$) insted of computing sqrtm, which is simply wrong. 

\begin{verbatim}
  As a result, instead of computing an expensive matrix square root, we can 
  do something much simpler, and has O(n) vs O(n^2) space complexity. 
\end{verbatim}

they compute trace\_sqrt\_product at line 716. 
They already have the proof in there .... 


\section{Conclusion}

==> sections/7_related_work.tex <==


\section{Related Work}
The literature contains several methods for evaluating generative models. 
An overview can be found in \cite{overview} which reviews a total of 29 different methods.
This article concerns the FID, which is arguably the most popular method, often used to benchmark state of the art generative models like, e.g., \cite{biggan}. 
%\am{Since we consider computational resources and adv example we cover that in rw below. ;; mention share code}

\label{sec:rw}
\subsection{Computational Resources}
To the best of our knowledge, there exists no published article which reduces the computational resources associated with the FID.  
However, some open-source implementations of FID contain modifications which remove parts of the resource heavy computations. 
% Such ``modified FIDs'' are faster but does not compute the right thing. 
Such ``modified FIDs'' are faster but resolves to approximations.
Below, we compare two modifications with our algorithm. 

\cite{meanfid} reduces time consumption from $O(d^3+d^2m)$ to $O(dm)$ by computing only $||\mu_1-\mu_2||_2^2$, omitting the trace term $\tr(\Sigma_1+\Sigma_2-2\sqrt{\Sigma_1\Sigma_2})$.   
\cite{diagfid} incorporates the covariance matrices while retaining the $O(dm)$ time complexity, by only using the diagonal entries of the covariance matrices. 
We emphasize that leaving out parts of the FID formula can introduce arbitrarily high levels of error. 
In comparison, our algorithm computes the exact FID in $O(d^2m)$ time.
%Our algorithm takes $O(d^2m)$ time but computes the exact FID. 
Even though our algorithm has a higher asymptotic time complexity, for $m\le 128$ it consumes no more than double the time of \cite{meanfid,diagfid}.
This is true because both algorithms compute Inception encodings which take more than half of the computation time. %since it spends less than $50\%$ of its time computing $||\mu_1-\mu_2||_2^2+\tr(\Sigma_1)+\tr(\Sigma_2)-2\cdot \tr(\sqrt{\Sigma_1\Sigma_2})$. 


Finally, \cite{eigfid} computes $\tr(\sqrt{\Sigma_1\Sigma_2})$ by computing the eigenvalues of $\sqrt{\Sigma_1}\Sigma_2\sqrt{\Sigma_1}$. 
This has the advantage that $\Sigma_1$ is symmetric so one can compute $\sqrt{\Sigma_1}$ through its eigendecomposition.
Such approach is not possible for $\Sigma_1\Sigma_2$ which, in general, is not symmetric. 
The derivations of \cite{eigfid} have some similarities to our derivations, but they do not exploit small $m$ and thus take $O(d^3+d^2m)$ time. 


\subsection{Adversarial Examples} 
The Inception Distance (ID) \cite{inceptiondistance} was widely used before the introduction of the FID. 
Previous work has successfully constructed adversarial examples against ID \cite{adversarialinception}. 
To the best of our knowledge, such adversarial examples have not been constructed for the FID. 
FastFID allows constructing such adversarial examples efficiently by simple gradient descent as presented in \Cref{sec:adv}. 

%\section{Code}
%To make FastFID and FastFCD widely accessible, we wrote a PyTorch implementation that computes FID and FCD by a single line of code, e.g., \textsc{fastfid(fake\_images)}. 
%Upon publication, we will make our implementation publicly available. 
%To further reproducibility, we attached an implementation of FastFID with accompanying test-cases in 'pythoncode.zip'. 
%To circumvent uploading pre-computed activations, we shared a variant that uses few ``real'' samples instead of the pre-computed activations. 
%The code can be run in Google Colab with automatic handling of dependencies. 

%https://github.com/tensorflow/tensorflow/blob/00fad90125b18b80fe054de1055770cfb8fe4ba3/tensorflow/contrib/gan/python/eval/python/classifier_metrics_impl.py#L411


%Types of evaluation of generive; inception score, wasserstein and fid. 

%Other approaches at speeding up FID computations. 


%Emperisk Wasserstein GANs;




==> sections/8_conclusion.tex <==


%\section{Future Work}
%In this work we demonstrated the mini-batch fake sample training of FID allow reducing validation FID evaluating using many samples. One would add additional information to the loss function if the fake samples was also $10k$, however, generating $10k$ samples in each iteration would simply take too long (reduce variance). 
%The increase in computation time could be alleviated by aggreagintg fake samples from previous iterations; e.g., with batch size 128 we could accumulate samples from the last 99 iterations and get a total of 12800 fake samples. The mean and covariance matries can be updated by accumulation fast, so the only thing one needs to update in each iteration is the trace matrix square root. This can be done using rank $k$ updates \cite{}, however, this is numerically unstable; we posit that this can be fixed, and training with such approach would reduce variance and improve relatiev to our approach. Notably, such training would heavily penalized generation of samples that are not varied. 



\section{Conclusion}
\label{sec:conclusion}
We introduced FastFID which computes FID fast when the number of ``real'' samples is large and the number of ``fake'' samples is small.
Depending on the number of ``fake'' samples, FastFID is between 25 to 500 times faster than a previous implementations. 
FastFID can be extended to the Frechet ChemNet Distance, FastFCD, which is between 30 to 150 times faster than a previous implementation. 
The attained speed-up is useful when evaluating FID/FCD frequently during training. 
Finally, FastFID
allow the construction of adversarial examples for FID by simple gradient descent.


**note; if it gets published. We suggest in the future that people report and compare generative models that are trained to explicitly minimize FID seperately from models that do minimize FID. Since running both such experiments is very time-consuming, we bla bla. 


\clearpage 

% ``fake'
%ffew number of "fakand backpropagation for FID.
%FastFID exploits a 

%Our implementation is between 25-500 times faster than \cite{}, Relative to a previous implementation, our , between 25-500 times faster than a previous implementation. 


%The Fréchet Inception Distance is arguably the most popular method. 
%In this article, we have demonstrated how to reduce computation time from $60s$ to $0.2s$. 
% it is also helpful in constructing adversarial examples for the Fréchet Inception Distance. 


==> tables/numerical_errors_simple.tex <==
\begin{table}[h]
    \caption{Numerical error of \textsc{scipy.linalg.sqrtm} and \Cref{algo:pseudocode} for different number of fake samples $m$. 
    We also report the ground truth so the percentage wise numerical error can be inferred. 
    }
    \label{fig:numerror}
    \centering
    \begin{tabular}{cccc}
    \toprule
         $m$ & Ground Truth & Error of \textsc{scipy.linalg.sqrtm} & Error of \Cref{algo:pseudocode} \\
    \midrule
% 8           & 14283.8174  & 175.1039   & 0.0000      \\
% 16          & 30678.9355  & 228.1520   & 0.0020      \\
 32          & 62955.6250  & 300.0112   & 0.0000      \\
 64          & 128947.5625 & 408.3399   & 0.0078     \\
 128         & 259586.1250 & 565.4011   & 0.0156      \\
 256         & 523360.3438 & 785.0262   & 0.0312     \\
    \bottomrule
    \end{tabular}
\end{table}
